Jacobi-Bernoulli cohomology and deformations of schemes and maps

We introduce a notion of Jacobi-Bernoulli cohomology associated to a semi-simplicial Lie algebra (SELA). For an algebraic scheme $X$ over $\C$, we construct a tangent SELA $\t_X$ and show that the Jacobi-Bernoulli cohomology of $\t_X$ is related to infinitesimal deformations of $X$.

==> myheader2.tex <==

\DeclareMathOperator{\RE}{Re}  \DeclareMathOperator{\IM}{Im}
\DeclareMathOperator{\diag}{Diag}
 \DeclareMathOperator{\ess}{ess}
 \DeclareMathOperator{\Zeros}{Zeros}
 \DeclareMathOperator{\Ideal}{Ideal}
 \DeclareMathOperator{\Spf}{Spf}
 \DeclareMathOperator{\Deff}{Deff}
 \DeclareMathOperator{\ext}{Ext}
 \DeclareMathOperator{\NCI}{NCI}
 \DeclareMathOperator{\norm}{{norm}}
\DeclareMathOperator{\Bl}{B\l} \DeclareMathOperator{\bl}{b\l}
\def\inv{^{-1}}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\xc}{XC}
%\DeclareMathOperator{\epp}{\epsilon}
%\DeclareMathOperator{\varepp}{\varepsilon}
\DeclareMathOperator{\del}{\partial}
\DeclareMathOperator{\Ext}{Ext} \DeclareMathOperator{\Hom}{Hom}
%\DeclareMathOperator{\red}{{red}}
\def\refp #1.{(\ref{#1})}
\renewcommand\theenumi{\roman{enumi}}
%\newcommand{\eps}{\varepsilon}
\newcommand{\bsl}{\begin{slide}{}}
\newcommand{\bes}{\begin{slide}{}\end{slide}}
\newcommand{\To}{\longrightarrow}
\newcommand{\h}{\mathcal{H}}
\newcommand{\cone}{\mathrm{cone}}
\newcommand{\st}{\ ^{\tilde{}}}
\newcommand{\s}{\mathcal{S}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\eps}{\epsilon}
%\newcommand{\c}{\mathcal }
\newcommand{\vareps}{\varepsilon}
\newcommand{\qis}{\sim_{\mathrm{qis}}}
\newcommand{\ba}{{\beta\alpha}}
\newcommand{\BOP}{\mathbf{B}}
\newcommand{\BH}{\mathbf{B}(\mathcal{H})}
\newcommand{\KH}{\mathcal{K}(\mathcal{H})}
\newcommand{\Real}{\mathbf{R}}
\newcommand{\Complex}{\mathbf{C}}
\newcommand{\Field}{\mathbf{F}}
\newcommand{\RPlus}{\Real^{+}}
\newcommand{\Polar}{\mathcal{P}_{\s}}
\newcommand{\Poly}{\mathcal{P}(E)}
\newcommand{\EssD}{\mathcal{D}}
\newcommand{\Lom}{\mathcal{L}}
\newcommand{\States}{\mathcal{T}}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\seq}[1]{\left<#1\right>}
%\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\essnorm}[1]{\norm{#1}_{\ess}}
%\newcommand{\Bbb}[1]{\mathbf #1}
%\newcommand{\mathfrak}[1]{\mathcal #1}
\newcommand{\Cal}[1]{\mathcal #1}
\newcommand{\act}[2]{\langle #1 , #2\rangle}
\newcommand{\legen}[2]{(\frac{#1}{#2})}
\newcommand{\un}{{\underline{n}}}
\newcommand{\ul}[1]{\underline {#1}}
\def\sch{\text{sch}}
\def\sbr #1.{^{[#1]}}
\def\sfl #1.{^{\lfloor #1\rfloor}}
\newcommand{\nred}{\ {^{\mathrm{red}}\mathcal{N}}}
\newcommand{\tred}{{\ ^{\mathrm{red}}\mathcal{T}}}
\newcommand{\ttt}{\tilde{\mathcal{T}}}
\newcommand{\tn}{\tilde{\mathcal{N}}}
\newcommand\col [2]
{\left[\begin{matrix}#1 \\ #2\end{matrix}\right]}
\newcommand\twostack [2]
{\begin{matrix}#1 \\ #2\end{matrix}}
\newcommand{\sectionend}
{\[\circ\gtrdot\ggg\mathbb{\times}\lll\lessdot\circ\]}
\newcommand\mat [4]
{\left[\begin{matrix}#1 &#2\\ #3 &#4\end{matrix}\right]}
\newcommand\limto [1] {\lim\limits_{\stackrel{\longrightarrow}
{#1}}}
\newcommand\adj {adj}
\newcommand\strad{{\mathrm {strad}}}
\newcommand\subp [1] {_{(#1)}}
\newcommand {\txp}{\t_X(P)}
\newcommand\jsh{\rm J^\sharp}
\newcommand\gb{\mathfrak g_\bullet}
\newcommand\half{\frac{1}{2}}
\newcommand\red{{\mathrm red}}
\def\bt{\boxtimes}
\def\what{\widehat}
\def\inv{^{-1}}
\def\?{{\bf{??}}}
\def\dgla{differential graded Lie algebra\ }
\def\dg{differential graded\ }
\def\Aut{\text{\rm Aut}}
\newcommand{\PGL}{\rm PGL}
\newcommand{\GL}{\rm GL}
\newcommand{\F}{\mathcal F}
\def\Ndr{N_d^{\text{red}}}
\def\Ndx{N_d^\times}
\def\Ndt{N_d^{\text{tac}}}
\def\Hilb{\text{Hilb}}
\def\fHilb{\text{fHilb}}
\def\Proj{\textrm{Proj}}
\def\RR{\mathcal R}
\def\H{\mathcal H}
\def\HH{\mathbb H}
\def\M{\Cal M}
\def\A{\Bbb A}
\def\X{\Cal X}
\def\E{\Cal E}
\def\F{\Cal F}
\def\Y{\Cal Y}
\def\SH{\Cal H}
\def\C{\mathbb C}
%\def\H{\Bbb H}
\def\P{\mathbb P}
%\def\F{\mathbb F}
\def\N{\mathbb N}
\def\R{\mathbb R}
\def\Z{\mathbb Z}
\def\bF{\mathbb{F}}
\def\Cz{\v{C}}
%\def\GL{{\text{ GL}}
\def\lb{\lambda}
\def\ord{\text{\rm ord}}
\def\sgn{\text{\rm sgn} }
\def\sym{\text{\rm sym} }
\def\Der{\text{\rm Der} }
\def\Spec{\text{\rm Spec} }
\def\ad{\text{\rm ad}}
\def\bp{\bar{\partial}}
\def\ls{\vskip.25in}
\def\ss{\vskip.12in}
\def\ms{\vskip.1in}
\def\Q{\mathbb Q}
%\def\[{\big[}
%\def\]{\big]}
\def\V{\bar{V}}
\def\L{\mathcal L}
\def\O{\mathcal O}
\def\UU{\mathcal U}
\def\y{\bar{y}}
\def\bt{\boxtimes}
\def\br{\text{br}}
\def\cob{^t\text{br}}
\def\Sym{\textrm{Sym}}
\def\id{\text{id}}
\def\rk{\text{rk}}
\def\Hi{\text{Hi}}
\def\hi{\text{hi}}
\def\g{\mathfrak g}
\def\J{\mathfrak J}
\def\gt{\tilde{\mathfrak g}}
\def\gh{\hat{\mathfrak g}}
\def\Et{\tilde{E}}
\def\Lt{\tilde{L}}
\def\gl{\mathfrak{gl}}
\def\sll{\mathfrak {sl}}
\def\h{\mathfrak h}
\def\rs{{\rho\sigma}}
\def\ab{{\alpha\beta}}
\def\bg{{\beta\gamma}}
\def\ga{{\gamma\alpha}}
\def\abg{{\alpha\beta\gamma}}
\def\m{\mathfrak m}
\def\k{\mathfrak k}
\def\endf{\mathfrak { end}}
\def\hom{\mathfrak {hom}}
\def\p{\partial}
\def\w{^\wedge}
\def\1/2{\frac{1}{2}}
\def\lmc{L_m(\C)}
\def\SD{\Cal S^{\text{v}}}
\def\gsh{\mathfrak g^\sharp}
\def\D{\mathfrak D}
\def\U{\mathfrak U}
\def\I{\mathcal{ I}}
\def\Y{\Cal Y}
\def\SS{\Cal S}
\def\Ann{\textrm{Ann}}
\def\Sec{\textrm{Sec}}
\def\nuline{\par\noindent}
\def\im{\text{im}}
\def\simto{\stackrel{\sim}{\rightarrow}}
\def\2{{[2]}}
\def\l{\ell}
\def\nl{\newline}
\def\n{\mathcal{N}}
\def\t{\mathcal{T}}
\def\Mbar{\overline{\mathcal M}}
\def\hom{\mathcal{H}\mathit{om}}
\def\RHom{\text{\rm R}\mathcal H\mathit om}
\def\That{\hat{T}}
%\def{\tn}{\tilde{\mathcal{N}}}
\def\<{\langle}
\def\>{\rangle}
\def\sela{SELA\ }
\def\endo{\mathcal{E}\mathit{nd}}
\def\nuline{\par\noindent}
\def\im{\text{im}}
%\def\simto{\overset{\sim}\to{\to}}
\def\2{{[2]}}
\def\l{\ell}
\def\Proj{\text{Proj}}
\def\sbr #1.{^{[#1]}}
\def\scl #1.{^{\lceil#1\rceil}}
\def\spr #1.{^{(#1)}}
\def\supp{\text{supp}}
\def\subpr#1.{_{(#1)}}

\renewcommand{\theequation}{\arabic{section}.\arabic{subsection}.\arabic{equation}}
\def\beq{\begin{equation*}}
\def\eeq{\end{equation*}}
\newcommand{\td}{\tilde }
\newcommand{\beqn}[1]{\begin{equation}#1\end{equation}}
\newcommand{\mex}[1]{\begin{example}\begin{rm}#1
\end{rm}
\end{example}}
\newcommand{\beql}[2]{\begin{equation}\label{#1}#2\end{equation}}
\newcommand{\beqa}[2]{\begin{eqnarray}\label{#1}#2\end{eqnarray}}
\newcommand{\eqspl}[2]{\begin{equation}\label{#1}
\begin{split}#2\end{split}\end{equation}}
\newcommand{\eqsp}[1]{\begin{equation*}
\begin{split}#1\end{split}\end{equation*}}
\newcommand{\itemul}[1]{\item[\underline{#1}]}
\newcommand{\exseq}[3]{
0\to #1\to #2\to #3\to 0
}
%\end{example}
%\end{rm}
\def\eex{\end{rm}\end{example}}
%\end{example}
%\end{example}
\newcommand\newsection[1]{\section{#1}\setcounter{equation}{0}
}
\newcommand\newsubsection[1]{\subsection{#1}\setcounter{equation}{0}}
\newcommand{\fJ}{\mathfrak J}
%\def\ber{\begin{rem} }
%\def\eer{ \end{rem}
%\end{comment}
% THEOREM ENV.
%---------------------------------------------------
\newtheorem*{mainthm}{Main Theorem}
\newtheorem{thm}{Theorem}[section]
\newtheorem{thmcon}[thm]{Theorem-Construction}
%\renewcommand{\thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{ex}{Exercise}[section]
\newtheorem{con}{Conjecture.}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{claim}[thm]{Claim}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{propdef}[thm]{Proposition-definition}
\newtheorem{defn}[thm]{Definition}%number together with conj
\theoremstyle{remark}
\newtheorem{ntn}{Notation}
\newtheorem{rem}[thm]{Remark}
\newtheorem{example}[thm]{Example}

\newcommand{\myrem}[1]{\begin{rem}\begin{rm}#1
\end{rm}
\end{rem}}
\newcommand{\mm}{m,m-1}
%\renewcommand{\thethm}{}  % unnumbered
\pagestyle{plain}
%\roman{theenumi}{i}
%%%
%--------------------------------------------------------------
%\pagestyle{myheadings} \markright{Semi-simplicial}
